Reward Maximization for Pure Exploration: Minimax Optimal Good Arm Identification for Nonparametric Multi-Armed Bandits

In multi-armed bandits, the tasks of reward maximization and pure exploration are often at odds with each other. The former focuses on exploiting arms with the highest means, while the latter may require constant exploration across all arms. In this work, we focus on good arm identification (GAI), a practical bandit inference objective that aims to label arms with means above a threshold as quickly as possible. We show that GAI can be efficiently solved by combining a reward-maximizing sampling algorithm with a novel nonparametric anytime-valid sequential test for labeling arm means. We first establish that our sequential test maintains error control under highly nonparametric assumptions and asymptotically achieves the minimax optimal e-power, a notion of power for anytime-valid tests. Next, by pairing regret-minimizing sampling schemes with our sequential test, we provide an approach that achieves minimax optimal stopping times for labeling arms with means above a threshold, under an error probability constraint. Our empirical results validate our approach beyond the minimax setting, reducing the expected number of samples for all stopping times by at least 50% across both synthetic and real-world settings.

==> discussion.tex <==
%Empirical and theoretical extensions to our work would include:
%1) tuning the density bound $c$ and convergence tolerance $\gamma, l(\cdot, \cdot)$ for preserving this method's theoretical guarantees,
%2) testing integral approximations in computation of kernel functions $K_0(\cdot, \cdot)$;
In this paper, we introduce KDPE, a new method for debiasing plug-in estimators that (i) does not require the IF as input, (ii) works as a general plug-in for any target parameters that satisfy our regularity conditions. Distinct from existing computational methods that aim to do IF-free debiasing, our approach does \emph{not} make any explicit attempt to approximate the IF, and retains the simplicity of a plug-in approach. 

Future work includes
(i) analyzing the effect of RKHS-norm regularization on the convergence and efficiency, (ii) finding simple heuristics for setting hyperparameters $c, \gamma, \lambda$, 
(iii) investigating how to apply sample-splitting and the extent to which it can relax our assumptions,
(iv) providing primitive conditions for RKHS approximation of the IF score equation (Assumption \ref{assump:S5}), and (v) verifying the validity of bootstrap.
% remains a key question, as well as 
Alternative methods for constructing confidence intervals include directly taking the quantiles of the bootstrap estimates and/or subsampling while bootstrapping, which we do not explore in Appendix \ref{app:simulation}.  The strong connection between our method and TMLE raises the question of whether TMLE variants, such as CTMLE \citep{coyle2023}, CV-TMLE \citep{book2011}, and one-step TMLE \citep{one_step_tmle}, can be adapted to KDPE to reduce computational costs. The empirical performance of KDPE for DGP2 also suggests that KDPE may provide better finite-sample performance. Understanding KDPE's effect on the behavior of the empirical process and second-order remainder terms are directions for future 
% theoretical
work.


==> minimax_lower_bounds.tex <==

Under parametric assumptions where distributions $P_a$ are parameterized by its mean $\mu_a$,  \cite{degenne2019pure} and  \cite{juneja2019samplecomplexitypartitionidentification} provide lower bounds on the sample complexity for THR and GAI under a fixed sampling scheme $\pi \in \Delta^K$.

\begin{theorem}[Asymptotic Instance-Dependent Lower Bound on Sample Complexity \citep{degenne2019pure}] \label{thm:parametric_samp_complex}
    % Assume that all arms Let $\xi \in [0,1]$ be a vector for thresholds for each arm, and let $\mu$ represent a vector of means. Then, 
    Let $P = \{P_a\}_{a \in [K]}$ be a set of distributions parameterized by their means $\mu_a$, where $\mu_a \neq \xi$ for all $a \in [K]$. Then, for THR, the lower bound on sample complexity for any algorithm with $\delta$-level error control is as follows:
    $$ \liminf_{\pi \in \Delta^K, \alpha \rightarrow 0} \frac{\EE_{\pi}[\tau_\text{stop}]}{\log(1/\delta)} \geq \sum_{a \in [K]} \frac{1}{d(\mu_a, \xi)}, $$
    where $d(x,y)$ denotes the KL-divergence between distributions with mean $x$ and $y$.

    Without loss of generality, assume there exists $g$ good arms, i.e. $|\Gcal_{\bm \mu}| = g$. For GAI, for any $i \leq g$, the limiting stopping time for labeling $i$ good arms under any algorithm with $\delta$-level error control is given by 
    $$\liminf_{\pi \in \Delta^K, \alpha \rightarrow 0} \frac{\EE_\pi[\tau_{\Gcal, i}]}{\log(1/\delta)} \geq \inf_{S \subseteq \{a \in [K]: \mu_a > \xi\}, |S| = i}\sum_{i \in S} \frac{1}{d(\mu_a, \xi)}.$$ 
\end{theorem}

These bounds are an immediate consequence of the optimality of likelihood ratio-based tests \citep{Wald1945SequentialTO} from the sequential testing literature. The restriction $\mu_a \neq \xi$ is to ensure that limits do not diverge to infinity. The lower bound on the stopping time for THR is simply obtained by using the optimal sequential test for each arm until it can be labeled as a good or bad arm. The lower bound for GAI is obtained by testing the $i$ arms with the shortest expected stopping times to determine $\mu_a > \xi$. 

Theorem \ref{thm:parametric_samp_complex} is well defined due to its parametric assumptions. The parametric setting naturally implies a corresponding distribution for the threshold value $\xi$, and allows divergence metrics to be well defined. In our fully nonparametric case, $\xi$ now corresponds to a highly composite distribution $\Pcal(\xi)$, where the divergence is no longer well-defined, and these bounds no longer hold. To provide a notion of optimality in our setting, we first introduce a class of sequential tests that (i) includes commonly used tests such as  likelihood-ratio based approaches and (ii) provide $\delta$-level error control under our nonparametric assumptions. 

\subsection{Anytime Valid Tests for Bounded Means} 
We leverage the modern theory of $e$-processes \citep{Ville1939, grunwald2020safe} in order to construct our sequential test and establish optimality. The $e$-process-based approach for $\delta$-level error control across $t \in \NN$ generalizes the likelihood ratio-based approaches that underlie the asymptotic lower bounds in Theorem \ref{thm:parametric_samp_complex}. We first define our class of $e$-processes below.


\begin{definition}[$e$-Processes for Non-parametric One-Sided Hypotheses]\label{defn:nonparam_e_process}
    Let $b \in [0,1]$ be a constant. For arm $a$ and null hypotheses $\Hcal^+_a = \{\Pcal(\mu_a): \mu_a > \xi\}$ and  $\Hcal^-_a = \{\Pcal(\mu_a): \mu_a \leq \xi\}$, we define a class of $e$-processes denoted as $\Ecal(\Hcal^+_a)$, $\Ecal(\Hcal^-_a)$ respectively:
    \begin{align}\label{eq:one_sided_test}
        % &
        \Ecal_t(\Hcal^-_a) = \{E_t(\lambda, \xi)\}_{\lambda \in [0, b/\xi]}, 
        \\
        \quad
        \Ecal_t(\Hcal_a^+) = \{E_t(\lambda, \xi)\}_{\lambda \in [-b/(1-\xi), 0]},
    \end{align} 
    where $E_t(\lambda, \xi) = \prod_{i: A_i = a} (1+  \lambda(X_i - \xi) )$ and $\lambda$ is a $\Fcal_{t-1}$-measurable univariate parameter. 
     
\end{definition}

\brian{add more explanation here about mechanics of $e$-process}

Using these $e$-processes, one obtains $\delta$-level error control for labeling a single arm $a$ as good (or bad) by checking whether the $e$-process $E_t \in \Ecal_t(\Hcal_a^-)$ (or $E_t \in \Ecal_t(\Hcal_a^+)$) is above $1/\delta$ at each time $t \in \NN$. 

\begin{prop}[$\delta$-level Error Control for $e$-Processes]\label{prop:delta_error_control}
    If $P_a \in \Hcal_a^+$, then for any  $E_t(\lambda, \xi) \in \Ecal_t(\Hcal_a^+)$, \begin{equation}\label{eq:error_control}
        \PP(\exists t \in \NN :  E_t(\lambda, \xi) \geq \frac{1}{\delta}) \leq \delta.
    \end{equation}
    Likewise, if $P_a \in \Hcal_a^-$, then for any $E_t(\lambda, \xi) \in \Ecal_t(\Hcal_a^-)$, Equation \ref{eq:error_control} holds. 
\end{prop}

Likelihood-based approaches are instances of an $e$-processes in the class $\Ecal_t(\Hcal_a^+)$ and $\Ecal_t(\Hcal_a^+)$.  Unlike likelihood-based sequential tests that require a common dominating measure, our class of $e$-processes provide $\delta$-level error control for arbitrary distributions, and enable inference for discrete, continuous, and/or mixture distribution null hypotheses, all encoded by the mean threshold value $\xi$.

\begin{remark}
    We note that our class of $e$-processes in Definition \ref{defn:nonparam_e_process} is a particular set of $e$-processes for bounded means called nonnegative test martingales. Nonnegative test martingales are an important subset of $e$-processes: any anytime valid procedure must utilize nonnegative test martingales to be admissible, in the sense defined by \cite{ramdas2022admissible}. When $b=1$, this class of $e$-processes is the \emph{universal} representation of all nonnegative test supermartingales under more general assumptions that only require conditional mean stationarity \citep{waudbysmith2022estimating}.
\end{remark}


To define our notion of optimality, we focus on the same class of sampling schemes $\pi \in \Delta^K$, but restrict our labeling rules to the class of sequential tests implied by the $e$-processes in Definition \ref{defn:nonparam_e_process}. We define $\Acal_{\Ecal}$ as the class of THR/GAI algorithms that use (i) sampling scheme $\pi \in \Delta^K$ and (ii) some choice of an $e$-process in $\Ecal_t(\Hcal_a^-)$, $\Ecal_t(\Hcal_a^+)$ to label arms. In the following section, we provide novel lower bounds on asymptotic optimality for THR/GAI over the algorithm class $\Acal_{\Ecal}$. 

\subsection{Minimax Asymptotic Optimality}

Under the class of algorithms $\Acal_{\epsilon}$, we present the minimax lower bounds on the expected stopping time for our approach. These minimax results first fix the mean of the bandit instance $\bm\mu$. Given the mean vector $\bm\mu$, our results lower bound the smallest possible stopping time with any algorithm in $\Acal_{\Ecal}$ for the worst case distribution $P \in \Pcal(\mu)$, the set of all bounded distributions with arm means $\bm\mu$. 

\begin{theorem}[Minimax Lower Bounds For Nonparametric Distributions]\label{thm:min_max_bound}
    Let $P \in \Pcal(\bm\mu)_{\bm\mu \in [0,1]^K\setminus \bm\xi}$ be a set of distributions parameterized by their means $\mu_a$, where $\mu_a \neq \xi$ for all $a \in [K]$. Let our THR algorithm be any algorithm in the class of algorithms $\Acal_{\Ecal}$. The worst-case lower bound on sample complexity for any algorithm with $\delta$-level error control is given by
    \begin{align}
        &\liminf_{\delta \rightarrow 0} \sup_{P \in \Pcal(\bm\mu)}\frac{\EE[\tau_{\text{stop}}]}{\log(1/\delta)} \geq \\ 
        & \quad \sum_{a \in [K]} \frac{1}{\log\frac{1-\mu_a}{1-\xi} + \mu_a \log\frac{\mu_a (1-\xi)}{\xi (1-\mu_a)}}.
    \end{align}

    Let our GAI algorithm be any algorithm in the class of algorithms $\Acal_{\Ecal}$. Without loss of generality, assume there exists $g$ good arms, and denote $\mu_{i^*}$ as the $i$-th largest mean in $\bm\mu$. For GAI, for any $i \leq g$, the limiting stopping time for labeling $i$ good arms in the worst case with $\delta$-level error control is given by
    \begin{align}
        &\liminf_{\delta \rightarrow 0} \sup_{P \in \Pcal(\bm\mu)}\frac{\EE[\tau_{\text{stop}}]}{\log(1/\delta)} \geq \\ 
        & \quad \sum_{a \in [K]: \mu_a \geq \mu_{i^*}} \frac{1}{\log\frac{1-\mu_a}{1-\xi} + \mu_a \log\frac{\mu_a (1-\xi)}{\xi (1-\mu_a)}}.
    \end{align}
\end{theorem}

These results closely mirror that of Theorem \ref{thm:parametric_samp_complex}, where the denominator term $d(\mu_a, \xi)$ is replaced with the divergence of two Bernoulli distributions with means $\mu_a$ and $\xi$. [Add some description of proof steps here.]


Given these lower bounds, our goal is to provide (i) $\Fcal_t$-measurable sequential tests used for labeling arms at each time $t$, and (ii) a sampling function $\pi: (A_i, X_i)_{i < t} \rightarrow \Delta^K$ that achieves the lower bounds shown in Theorem \ref{thm:min_max_bound}. We first provide our novel sequential tests, which generalizes the Bernoulli likelihood ratio to the nonparametric setting while maintaining $\delta$-level error control. 


